ChatSplat: 3D Conversational Gaussian Splatting

Humans naturally interact with their 3D surroundings using language, and modeling 3D language fields for scene understanding and interaction has gained growing interest. This paper introduces ChatSplat, a system that constructs a 3D language field, enabling rich chat-based interaction within 3D space. Unlike existing methods that primarily use CLIP-derived language features focused solely on segmentation, ChatSplat facilitates interaction on three levels: objects, views, and the entire 3D scene. For view-level interaction, we designed an encoder that encodes the rendered feature map of each view into tokens, which are then processed by a large language model (LLM) for conversation. At the scene level, ChatSplat combines multi-view tokens, enabling interactions that consider the entire scene. For object-level interaction, ChatSplat uses a patch-wise language embedding, unlike LangSplat's pixel-wise language embedding that implicitly includes mask and embedding. Here, we explicitly decouple the language embedding into separate mask and feature map representations, allowing more flexible object-level interaction. To address the challenge of learning 3D Gaussians posed by the complex and diverse distribution of language embeddings used in the LLM, we introduce a learnable normalization technique to standardize these embeddings, facilitating effective learning. Extensive experimental results demonstrate that ChatSplat supports multi-level interactions -- object, view, and scene -- within 3D space, enhancing both understanding and engagement.

==> tab/lerf_obj.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{lccc}
    \toprule
    \textbf{Method} & \textbf{teatime} & \textbf{ramen} & \textbf{Mean} \\
    \midrule
    LLaVA-OV & 81.33 & 83.62 & 82.48 \\
    ChatSplat & 84.17 & 83.53 & 83.85 \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of methods for teatime and ramen with their mean scores.}
    \label{tab:lerf_obj}
\end{table}

==> tab/replica_obj.tex <==
\begin{table}[h!]
    \small
    \centering
    \begin{tabular}{lccccc}
    \toprule
    \textbf{Method} & \textbf{room\_0} & \textbf{room\_1} & \textbf{office\_2} & \textbf{office\_3} & \textbf{Mean} \\
    \midrule
    LLaVA-OV & 81.33 & 83.62 & 85.00 & 83.12 & 83.27 \\
    ChatSplat & 84.17 & 83.53 & 85.53 & 84.06 & 84.32 \\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Quantitative Results on the Replica Dataset at Object Level.} On the more complex indoor Replica dataset, our approach continues to outperform the baseline across most scenes and overall.}
    \label{tab:replica_obj}
\end{table}
